Generalized van Trees inequality: Local minimax bounds for non-smooth functionals and irregular statistical models

In a decision-theoretic framework, the minimax lower bound provides the worst-case performance of estimators relative to a given class of statistical models. For parametric and semiparametric models, the H\'{a}jek--Le Cam local asymptotic minimax (LAM) theorem provides the sharp local asymptotic lower bound. Despite its relative generality, this result comes with limitations as it only applies to the estimation of differentiable functionals under regular statistical models. On the other hand, minimax lower bound techniques such as Fano's or Assoud's are applicable in more general settings but are not sharp enough to imply the LAM theorem. To address this gap, we provide new non-asymptotic minimax lower bounds under minimal regularity assumptions, which imply sharp asymptotic constants. The proposed lower bounds do not require the differentiability of functionals or regularity of statistical models, extending the efficiency theory to broader situations where standard results fail. The use of the new lower bounds is illustrated through the local minimax lower bound constants for estimating the density at a point and directionally differentiable parameters.

==> main/directional_derivative.tex <==
\section{Application to Gateaux differentiable functionals}
\subsection{Van Trees inequality for non-smooth functionals}
Lemma~\ref{lm:crvtBound} removes often required differentiablity assumptions over both functional $\psi$ and statistical models $\{P_\theta : \theta \in \Theta \}$. We can simplify the lower bound significantly by assuming the standard regularity to one of them. In this section, we present the result for the lower bound associated with estimating a non-smooth functional under a regular statistical model. 

We first introduce several notations. For a density function $g$ with the support $T$ such that $g=0$ on its boundary, we define the Fisher information of $g$ as 
\begin{align*}
    \mathcal{J}(g) = \int_T \frac{\nabla g(t)\nabla g(t)^T}{g(t)}I\{g(t)>0\}\,dt.
\end{align*}

Next, we define Hellinger differentiability, which we later assume that the statistical model in question satisfies. 
\begin{definition}[Hellinger differentiability] A statistical model $\{P_\theta : \theta \in \Theta\}$ is Hellinger differentiable at $\theta_0 \in \Theta$
if there exists a real-valued function $\dot{\xi}_{0} \in L_2(\mu)$ such that
\begin{align}
    \|f_{\theta_0+h}^{1/2} - f_{\theta_0}^{1/2} - h\dot{\xi_0}\|_{\mu} = o(|h|) \qquad \text{ as } h \longrightarrow 0
\end{align}
We then define the Fisher information $\mathcal{I}(\theta_0)$ of the model at $\theta$ as 
\begin{align}
    \mathcal{I}(\theta_0) \coloneqq 4 \int_{\mathcal{X}} \dot{\xi}_0\dot{\xi}_0^T\, d\mu
\end{align}
\end{definition}
We present the following regularity conditions over the statistical model.
\begin{enumerate}[label=\textbf{(A\arabic*)}]
\setcounter{enumi}{2}
    \item \label{as:hellinger} The statistical model $\{P_\theta : \theta \in \Theta\}$ is Hellinger differentiable at $\theta_0 \in \Theta$.
    \item \label{as:ac_model}The mapping $(x, \theta) \in \mathcal{X}\times\Theta \mapsto f_\theta(x)$ is measurable and the function $\theta \in \Theta \mapsto f_\theta(x)$ is absolutely continuous for $\mu$-almost everywhere with the partial derivative at $\theta$ denoted by $\nabla f_\theta(x)$. Furthermore, $\nabla f_\theta(x)I\{f_\theta>0\}/\sqrt{f_\theta}$ belongs to $L_2(\mu)$ for $\mu$ almost everywhere.
\end{enumerate}
We now state the following lower bound for non-smooth functionals.
% If each base model $\{P_\theta\}_{\theta\in\Theta}$ satisfies \ref{as:hellinger}, then the product model $\{P^n_\theta\}_{\theta\in\Theta}$ also satisfies \ref{as:hellinger} with the derivative 
% \[(x_1, x_2, \dots, x_n) \mapsto \sum_{i=1}^n \dot{\xi}_{\theta}(x_i)\prod_{i\neq j} \xi_{\theta}(x_j)\]
% and the Fisher information of the product model at $\theta_0$ becomes $n\mathcal{I}(\theta_0)$. We now state the following corollary to Theorem~\ref{thm:general_vt_inequality}.
% \begin{corollary}\label{cor:vt_inequality}
% If \ref{as:hellinger}--\ref{as:ac_model} hold, then the statement of Theorem~\ref{thm:general_vt_inequality} simplifies as follows;
% \begin{align*}
%   & \sup_{|t|<1} \E^n_{\theta_0 + tc/n^{1/2}}\left[n^{1/2}\left\{S_n(x)-\psi(\theta_0+tc/n^{1/2})\right\}\right]^2\\
%   &\qquad \geq \sup_{g}\sup_{ \{h : |h|=1\}}\frac{\lim_{\varepsilon\downarrow 0}\left[\int_{-1}^1\epsilon^{-1}\left\{\psi(\theta_0+ tc/n^{1/2})-\psi(\theta_0+ tc/n^{1/2}-h\varepsilon)\right\}g(t)\, dt\right]^2}{\frac{1}{c^2}\mathcal{J}(g)+\int_{-1}^1\mathcal{I}(\theta_0 + tc/n^{1/2})g(t)\,dt}.
% \end{align*}
% \end{corollary}
\begin{lemma}[van Trees inequality for Gateaux differentiable functionals \kt{name?}]
\label{lm:vtBound_directional} Suppose $q$ is a density function that satisfies \ref{as:IPBorder}. In addition, we assume $g$ has following properties; (i) It is bounded and absolutely continuous; (ii) It tends to zero towards the boundary of its support; (iii) The Fisher information is finite. Then for a real-valued functional $\psi$, we have
\begin{align*}
   & \inf_{S_n}\int_{\Theta}\E_{\theta}\left\{S_n(x)-\psi(\theta)\right\}^2q(\theta)\, d\lambda\geq  \sup_{\{h:\|h\|=1\}}\lim_{\varepsilon \downarrow 0}\frac{\left\{\int_{\Theta}\varepsilon^{-1} \left(\psi(\theta)-\psi(\theta-h\varepsilon)\right)q(\theta)\,d\lambda\right\}^2}{ h^T \mathcal{J}(q)h + A(\varepsilon, h, q, f_{\theta})}.
\end{align*}
where 
\begin{align*}
    A(\varepsilon, h, q, f_{\theta}) \coloneqq \varepsilon^{-2}\iint_{\mathcal{X}\times \Theta} \frac{q(\theta+h\varepsilon)^2}{q(\theta)}\frac{\left\{f_{\theta+h\varepsilon}(x)-f_\theta(x)\right\}^2}{f_\theta(x)}I(q(\theta)f_\theta(x) > 0)\,d\mu(x)\,d\lambda.
\end{align*}
Additionally, if \ref{as:hellinger}--\ref{as:ac_model} hold, we have
\begin{align*}
   & \inf_{S_n}\int_{\Theta}\E_{\theta}\left\{S_n(x)-\psi(\theta)\right\}^2q(\theta)\, d\lambda\geq  \sup_{\{h:\|h\|=1\}}\frac{\lim_{\varepsilon \downarrow 0}\left\{\int_{\Theta}\varepsilon^{-1} \left(\psi(\theta)-\psi(\theta-h\varepsilon)\right)q(\theta)\,d\lambda\right\}^2}{ h^T \left(\mathcal{J}(q) + \int_{\Theta} q(\theta) \mathcal{I}(\theta)\,d\lambda\right) h}.
\end{align*}
\end{lemma}

\begin{proof}[\bfseries{Proof of Lemma~\ref{lm:vtBound_directional}}]
The proof of Lemma~\ref{lm:vtBound_directional} is a direct application of Lemma~\ref{lm:crvtBound} by replacing $h$ in the bound with a convergent sequence of $h\varepsilon_n$ such that $\varepsilon_n \downarrow 0$ and $\|h\|=1$. We now define the notation for Gateaux derivatives. 
\begin{definition}[Gateaux derivative]
A vector-valued functional $\psi \coloneqq \Theta \mapsto \mathbb{R}^k$ is said to be Gateaux differentiable at $\theta_0 \in \Theta$ if for fixed $h \in \Theta$ there exists a mapping $\psi'_\theta(h)$ such that
\begin{align*}
    \left\|\frac{\psi(\theta_0+th) - \psi(\theta_0)}{t} - \psi'_{\theta_0}(h) \right\| = o(1) \qquad \text{as } t\longrightarrow0.
\end{align*}
\end{definition}
The above definition is equivalent to the following;
\[\psi(\theta_0+th) - \psi(\theta_0) = t\psi'_{\theta_0}(h) + o(t)  \qquad \text{as } t\longrightarrow0.\]
If a function is differentiable at $\theta$, then we have $\psi'_\theta(h) = \nabla \psi(\theta) h$ where $\nabla \psi(\theta) \in \mathbb{R}^k \times \Theta$. \kt{Though confusing, $\nabla \psi(\theta)^T h$ is more appropriate for a real-valued function where $\nabla \psi(\theta)$ is conventionally a column vector.}

Suppose $h\in \Theta$ is a fixed vector with $\|h\|=1$ and $\|h\varepsilon_n\| < \delta$. Then by applying Lemma~\ref{lm:crvtBound}, we have
\begin{align*}
   & \inf_{S}\int_{\Theta}\E_{\theta}\left\{S(x)-\psi(\theta)\right\}^2q(\theta)\, d\lambda \\
   &\qquad \geq  \lim_{\varepsilon_n\downarrow 0}\frac{\left\{\int_{\Theta} \left(\psi(\theta)-\psi(\theta-h\varepsilon_n)\right)q(\theta)\,d\lambda\right\}^2}{\int_\Theta\frac{\left\{q(\theta+h\varepsilon_n)-q(\theta)\right\}^2}{q(\theta)}I(q(\theta)>0)\,d\lambda+\iint_{\mathcal{X}\times \Theta} \frac{q(\theta+h\varepsilon_n)^2}{q(\theta)}\frac{\left\{f_{\theta+h\varepsilon_n}(x)-f_\theta(x)\right\}^2}{f_\theta(x)}I(q(\theta)f_\theta(x) > 0)\,d\mu(x)\,d\lambda}
\end{align*}
We now analyze each term in the above display. For the first term of the denominator, we have
\begin{align*}
    \lim_{\varepsilon_n\downarrow0}\int_\Theta\frac{\left\{q(\theta+h\varepsilon_n)-q(\theta)\right\}^2}{q(\theta)}I(q(\theta)>0)\,d\lambda &= \int_\Theta\frac{\left\{\varepsilon q'_\theta(h) + o(\varepsilon)\right\}^2}{q(\theta)}I(q(\theta)>0)\,d\lambda\\
    &=\varepsilon ^2 \int_\Theta\frac{\left\{\nabla q(\theta)^Th \right\}^2}{q(\theta)}I(q(\theta)>0)\,d\lambda + o(\varepsilon^2)\\
    &=\varepsilon ^2 \int_\Theta\frac{h^T\nabla q(\theta)\nabla q(\theta)^Th }{q(\theta)}I(q(\theta)>0)\,d\lambda + o(\varepsilon^2)\\
    &=\varepsilon^2 h^T\mathcal{J}(q)h + o(\varepsilon^2)
\end{align*}
where we used the dominated convergence theorem, the definition of Gateaux derivative, the definition of absolute continuity, and the definition of the Fisher information. We conclude the first statement by the multiplication and division of the lower bound with $\varepsilon_n^{-2}$ and taking the supremum over $h$. 

For the second statement, we show that the second term of the denominator can be further simplified in view of \ref{as:hellinger} and \ref{as:ac_model}. By the similar derivation as above, we have

\begin{align*}
&\lim_{\varepsilon_n\downarrow 0}\iint_{\mathcal{X}\times \Theta} \frac{q(\theta+h\varepsilon_n)^2}{q(\theta)}\frac{\left\{f_{\theta+h\varepsilon_n}(x)-f_\theta(x)\right\}^2}{f_\theta(x)}I(q(\theta)f_\theta(x) > 0)\,d\mu(x)\,d\lambda\\
&\qquad = \lim_{\varepsilon_n\downarrow 0}\int_\Theta \frac{\{q(\theta+h\varepsilon_n)-q(\theta)+q(\theta)\}^2}{q(\theta)}I(q(\theta)>0)\int_{\mathcal{X}} \frac{\left\{f_{\theta+h\varepsilon_n}(x)-f_\theta(x)\right\}^2}{f_\theta(x)}I(f_\theta(x) > 0)\,d\mu(x)\,d\lambda\\
&\qquad = \lim_{\varepsilon_n\downarrow 0}\int_\Theta \{q(\theta)+O(\varepsilon)\}I(q(\theta)>0)\int_{\mathcal{X}} \frac{\left\{f_{\theta+h\varepsilon_n}(x)-f_\theta(x)\right\}^2}{f_\theta(x)}I(f_\theta(x) > 0)\,d\mu(x)\,d\lambda\\
&\qquad =\int_\Theta \{q(\theta)+O(\varepsilon)\}I(q(\theta)>0)\int_{\mathcal{X}} \lim_{\varepsilon_n\downarrow 0} \frac{\left\{f_{\theta+h\varepsilon_n}(x)-f_\theta(x)\right\}^2}{f_\theta(x)}I(f_\theta(x) > 0)\,d\mu(x)\,d\lambda\\
&\qquad =\int_\Theta \{q(\theta)+O(\varepsilon)\}I(q(\theta)>0)\int_{\mathcal{X}} \frac{\left\{\varepsilon_n f'_{\theta}(h)+o(\varepsilon_n)\right\}^2}{f_\theta(x)}I(f_\theta(x) > 0)\,d\mu(x)\,d\lambda\\
&\qquad =\varepsilon_n^2\int_\Theta q(\theta)\int_{\mathcal{X}} \frac{\left(\nabla f_{\theta}^Th\right)^2}{f_\theta(x)}I(f_\theta(x) > 0)\,d\mu(x)\,d\lambda + O(\varepsilon_n^3) + o(\varepsilon_n^2)\\
&\qquad =\varepsilon_n^2\int_\Theta q(\theta)\int_{\mathcal{X}} \frac{h^T\nabla f_{\theta}\nabla f_{\theta}^Th}{f_\theta(x)}I(f_\theta(x) > 0)\,d\mu(x)\,d\lambda + o(\varepsilon_n^2)\\
&\qquad = \varepsilon^2h^T \left(\int_{\Theta} q(\theta) \mathcal{I}(\theta)\,d\lambda\right) h+ o(\varepsilon^2)
\end{align*}
where we used uniform continuity of $q$, the dominated convergence \kt{check}, the definition of Gateaux derivative \kt{check}, Lemma~\ref{lm:dqm_and_fisher_info} \kt{check}. 
% \kt{Check swapping the limit and integration. I think we need slightly stronger. Something like local boundedness of $f$. I also think we need to improve Lemma~\ref{lm:dqm_and_fisher_info} to account for directional differentiable almost everywhere (I think the proof already works for every directions)}.
Putting together, the denominator of the lower bound becomes
\begin{align*}
    &\int_\Theta\frac{\left\{q(\theta+h)-q(\theta)\right\}^2}{q(\theta)}I(q(\theta)>0)\,d\lambda+\iint_{\mathcal{X}\times \Theta} \frac{q(\theta+h)^2}{q(\theta)}\frac{\left\{f_{\theta+h}(x)-f_\theta(x)\right\}^2}{f_\theta(x)}I(q(\theta)f_\theta(x) > 0)\,d\mu(x)\,d\lambda \\
    &\qquad = \varepsilon^2 h^T \left(\mathcal{J}(q) + \int_{\Theta} q(\theta) \mathcal{I}(\theta)\,d\lambda\right) h+ o(\varepsilon^2).
\end{align*}
Thus we conclude the second statement by the multiplication and division of the lower bound with $\varepsilon_n^{-2}$ and taking the supremum over $h$. 
\end{proof}

\subsection{Local asymptotic minimax lower bounds for non-smooth functionals}
In this section, we demonstrate the application of Lemma~\ref{lm:vtBound_directional} to local asymptotic minimax lower bounds for the square risk in parametric models. Suppose we observe $n$ IID sequence $X_1, X_2, \dots, X_n$ from a statistical model $P_{\theta_0} \in \{P_\theta : \theta \in \Theta\}$. For simplicity, we assume the functional of interest $\psi$ is a real-valued mapping $\Theta \mapsto \mathbb{R}$ and let $S_n$ be an estimator of $\psi(\theta_0)$, which is a function of $X_1, X_2, \dots, X_n$. We denote by $\E^n_{\theta}$ the expectation relative to the sequence of statistical models $\left\{(P^n_\theta)_{\theta\in\Theta}\right\}_{n\geq 1}$. If each base model $\{P_\theta\}_{\theta\in\Theta}$ satisfies \ref{as:hellinger}, then the product model $\{P^n_\theta\}_{\theta\in\Theta}$ also satisfies \ref{as:hellinger} with the derivative 
\[(x_1, x_2, \dots, x_n) \mapsto \sum_{i=1}^n \dot{\xi}_{\theta}(x_i)\prod_{i\neq j} \xi_{\theta}(x_j)\]
and the Fisher information of the product model at $\theta_0$ becomes $n\mathcal{I}(\theta_0)$. We now present the following result.
\begin{lemma}[Local asymptotic minimax lower bounds for non-smooth functionals]\label{lm:lam_directional} 
Suppose $g$ is a density function with following properties; (i) It is bounded and absolutely continuous; (ii) The support is contained in $(-1,1)$ and $g(-1)=g(1)=0$ (iii) The Fisher information is finite. 
For any $c > 0$ and any sequences $\{S_n\}$ of estimators, we have
% \begin{align*}
%   & \inf_{S_n}\sup_{|t|<1} \E^n_{\theta_0 + tc/n^{1/2}}\left\{S_n(x)-\psi(\theta_0+tc/n^{1/2})\right\}^2 \\
%   &\qquad \geq \sup_{g}\sup_{ \{h : |h|=1\}}\frac{\lim_{\varepsilon\downarrow 0}\left[\int_{-1}^1\epsilon^{-1}\left\{\psi(\theta_0+ tc/n^{1/2})-\psi(\theta_0+ tc/n^{1/2}-h\varepsilon)\right\}g(t)\, dt\right]^2}{\frac{n}{c^2}\mathcal{J}(g)+\lim_{\varepsilon \downarrow 0} A(\varepsilon, h, g, f_{\theta_0+tc/n^{1/2}})} \\
%   &\text{ where }\, A(\varepsilon, h, g, f_\theta) \coloneqq \int_{-1}^{1}\frac{g(t+n^{1/2}h\varepsilon/c)^2}{g(t)}I\{g(t) > 0\}\int_{\mathcal{X}} \frac{\left\{f_{\theta+h\varepsilon}(x)-f_{\theta}(x)\right\}^2}{\varepsilon^2 f_{\theta}(x)}I\{f_{\theta}(x) > 0\}\,d\mu(x)\,dt
% \end{align*}
\begin{align*}
&\inf_{S_n}\sup_{|t|<1} \E^n_{\theta_0 + tc/n^{1/2}}\left\{S_n(x)-\psi(\theta_0+tc/n^{1/2})\right\}^2\\
   &\qquad\geq  \sup_g \sup_{\{h:\|h\|=1\}}\lim_{\varepsilon \downarrow 0}\frac{\left\{\int_{-1}^1 \varepsilon^{-1}\{\psi(\theta_0+tc/n^{1/2})-\psi(\theta_0+tc/n^{1/2}-h\varepsilon)\}g(t)\,dt\right\}^2}{ h^T \frac{n}{c^2}\mathcal{J}(g)h + A(\varepsilon, h, q_{n,c}, f_{\theta})}
\end{align*}
where
\begin{align*}
A(\varepsilon, h, q_{n,c}, f_{\theta})
    & = \int_{-1}^1\frac{g(t+n^{1/2}h\varepsilon/c)^2}{g(t)}I\{g(t) > 0\}\\
    &\qquad\qquad\int_{\mathcal{X}} \frac{\left\{f_{\theta_0+tc/n^{1/2}+h\varepsilon}(x)-f_{\theta_0+tc/n^{1/2}}(x)\right\}^2}{\varepsilon^2 f_{\theta_0+tc/n^{1/2}}(x)}I\{f_{\theta_0+tc/n^{1/2}}(x) > 0\}\,d\mu(x)\,dt.
\end{align*}
Additionally if \ref{as:hellinger}--\ref{as:ac_model} hold, then we have
% \begin{align*}
%   & \inf_{S_n}\sup_{|t|<1} \E^n_{\theta_0 + tc/n^{1/2}}\left[n^{1/2}\left\{S_n(x)-\psi(\theta_0+tc/n^{1/2})\right\}\right]^2\\
%   &\qquad \geq \sup_{g}\sup_{ \{h : |h|=1\}}\frac{\lim_{\varepsilon\downarrow 0}\left[\int_{-1}^1\epsilon^{-1}\left\{\psi(\theta_0+ tc/n^{1/2})-\psi(\theta_0+ tc/n^{1/2}-h\varepsilon)\right\}g(t)\, dt\right]^2}{\frac{1}{c^2}\mathcal{J}(g)+\int_{-1}^1\mathcal{I}(\theta_0 + tc/n^{1/2})g(t)\,dt}.
% \end{align*}
\begin{align*}
    & \inf_{S_n}\sup_{|t|<1} \E^n_{\theta_0 + tc/n^{1/2}}\left\{S_n(x)-\psi(\theta_0+tc/n^{1/2})\right\}^2\\
   &\qquad\geq  \sup_{\{h:\|h\|=1\}}\frac{\left\{\int_{-1}^1 \varepsilon^{-1}\{\psi(\theta_0+tc/n^{1/2})-\psi(\theta_0+tc/n^{1/2}-h\varepsilon)\}g(t)\,dt\right\}^2}{ nh^T \left(\frac{1}{c^2}\mathcal{J}(g) + \int_{-1}^1  \mathcal{I}(\theta_0 + tc/n^{1/2})g(t)\,dt\right) h}.
\end{align*}
\end{lemma}
\begin{proof}[\bfseries{Proof of Lemma~\ref{lm:lam_directional}}]
Throughout the proof, we treat $c > 0$ as a fixed constant. We define a random variable $T \in \Theta \subseteq \mathbb{R}^p$ whose support is contained in a $p$-dimensional open ball with radius one. The distribution of $T$ is given by a bounded and absolutely continuous density function $g := \Theta \mapsto \mathbb{R}^+$ with $g(\cdot) = 0$ for all $t \notin \mathcal{B}_p([0], 1)$. Additionally, we define a random variable $\theta_0 + cT/\sqrt{n}$ whose density is given by $q_{n,c}$. By the change of variables, we have 
\begin{align*}
    q_{n,c}(u) = \frac{d}{du} P(\theta_0 + cn^{-1/2}t \leq u) = \frac{d}{du}P\left(t \leq \frac{n^{1/2}(u-\theta_0)}{c}\right) = \frac{n^{1/2}}{c}g\left(\frac{n^{1/2}(u-\theta_0)}{c}\right).
\end{align*}
Therefore the absolute continuity of $g$ implies the absolute continuity of $q_{n,c}$. By a similar application of the change of variables, we have
\begin{align*}
    \mathcal{J}(q_{n,c}) &= \int_{\Theta} \frac{\nabla q_{n,c}(u)\nabla q_{n,c}(u)^T}{q_{n,c}(u)} I(q_{n,c}(u) > 0)\, du \\
    &= \int_{\Theta} \frac{n^{1/2}}{c}\frac{\nabla g \left((u-\theta_0)\frac{n^{1/2}}{c}\right)\nabla g \left((u-\theta_0)\frac{n^{1/2}}{c}\right)^T}{g\left((u-\theta_0)\frac{n^{1/2}}{c}\right)}I\left\{g\left((u-\theta_0)\frac{n^{1/2}}{c}\right) > 0\right\}\,du \\
    &= \int_{\Theta} \frac{n}{c^2}\frac{\nabla g(t)\nabla g(t)^T}{g(t)}I(g(t)>0)\, dt \\
    &= \frac{n}{c^2} \mathcal{J}(g).
\end{align*}
Therefore, $\mathcal{J}(g) < \infty$ implies $\mathcal{J}(q_{n,c}) < \infty$. We now apply Lemma~\ref{lm:lam_directional} to the density $q_{n,c}$. The required condition \ref{as:IPBorder} is trivially satisfied since the support of $q_{n,c}$ is an open set $(\theta_0-c/\sqrt{n}, \theta_0+c/\sqrt{n})$, which is eventually contained in $\Theta$ for $n$ large enough assuming $\Theta$ is open. Lemma~\ref{lm:vtBound_directional} then implies
\begin{align*}
   & \inf_{S_n}\int_{\Theta}\E^n_{\theta}\left\{S_n(x)-\psi(\theta)\right\}^2q_{n,c}(\theta)\, d\lambda\geq  \sup_{\{h:\|h\|=1\}}\lim_{\varepsilon \downarrow 0}\frac{\left\{\int_{\Theta}\varepsilon^{-1} \left(\psi(\theta)-\psi(\theta-h\varepsilon)\right)q_{n,c}(\theta)\,d\lambda\right\}^2}{ h^T \frac{n}{c^2}\mathcal{J}(g)h + A(\varepsilon, h, q_{n,c}, f_{\theta})}.
\end{align*}
We can first manipulate the upper-bound by the change of variables with $t=n^{1/2}(\theta-\theta_0)/c$,
\begin{align*}
   \int_{\Theta}\E^n_{\theta}\left(S_n(x)-\psi(\theta)\right)^2q_{n,c}(\theta)\, d\lambda &= \int_{-1}^1 \E^n_{\theta_0 + tc/n^{1/2}}\left\{S_n(x)-\psi(\theta_0+tc/n^{1/2})\right\}^2g(t)\, dt \\
   & \leq \sup_{|t|<1} \E^n_{\theta_0 + tc/n^{1/2}}\left\{S_n(x)-\psi(\theta_0+tc/n^{1/2})\right\}^2.
\end{align*}
Next, we analyze the lower-bound. By the change of variable with $\theta = \theta_0 + tcn^{-1/2}$, the numerator of the right-hand-side term in the above display becomes
\begin{align*}
\left\{\int_{\Theta}\varepsilon^{-1}( \psi(\theta)-\psi(\theta-h\varepsilon))q_{n,c}(\theta)\,d\theta\right\}^2 &= \left\{\int_{-1}^1 \varepsilon^{-1}\{\psi(\theta_0+tc/n^{1/2})-\psi(\theta_0+tc/n^{1/2}-h\varepsilon)\}g(t)\,dt\right\}^2.
\end{align*}
Furthermore, the second term of the denominator becomes 
\begin{align*}
    A(\varepsilon, h, q_{n,c}, f_{\theta})&= \varepsilon^{-2}\iint_{\mathcal{X}\times \Theta} \frac{q_{n,c}(\theta+h\varepsilon)^2}{q_{n,c}(\theta)}\frac{\left\{f_{\theta+h\varepsilon}(x)-f_\theta(x)\right\}^2}{f_\theta(x)}I(q_{n,c}(\theta)f_\theta(x) > 0)\,d\mu(x)\,d\lambda\\
    & = \int_{-1}^1\frac{g(t+n^{1/2}h\varepsilon/c)^2}{g(t)}I\{g(t) > 0\}\\
    &\qquad\qquad\int_{\mathcal{X}} \frac{\left\{f_{\theta_0+tc/n^{1/2}+h\varepsilon}(x)-f_{\theta_0+tc/n^{1/2}}(x)\right\}^2}{\varepsilon^2 f_{\theta_0+tc/n^{1/2}}(x)}I\{f_{\theta_0+tc/n^{1/2}}(x) > 0\}\,d\mu(x)\,dt.
\end{align*}
% \kt{To discuss: how far should I simplify? If it's reasonable to assume $f$ is locally bounded in a small neighborhood of $\theta_0$, then by the dominated convergence theorem,
% \begin{align*}
%     &\lim_{\varepsilon \downarrow 0}   \int_{-1}^1\frac{g(t+n^{1/2}h\varepsilon/c)^2}{g(t)}I\{g(t) > 0\}\\
%     &\qquad\qquad\int_{\mathcal{X}} \frac{\left\{f_{\theta_0+tc/n^{1/2}+h\varepsilon}(x)-f_{\theta_0+tc/n^{1/2}}(x)\right\}^2}{\varepsilon^2f_{\theta_0+tc/n^{1/2}}(x)}I\{f_{\theta_0+tc/n^{1/2}}(x) > 0\}\,d\mu(x)\,dt\\
%     &=\int_{-1}^1\lim_{\varepsilon \downarrow 0}\frac{g(t+n^{1/2}h\varepsilon/c)^2}{g(t)}I\{g(t) > 0\}\\
%     &\qquad\qquad\int_{\mathcal{X}} \frac{\left\{f_{\theta_0+tc/n^{1/2}+h\varepsilon}(x)-f_{\theta_0+tc/n^{1/2}}(x)\right\}^2}{\varepsilon^2f_{\theta_0+tc/n^{1/2}}(x)}I\{f_{\theta_0+tc/n^{1/2}}(x) > 0\}\,d\mu(x)\,dt\\
%     &=\int_{-1}^1\lim_{\varepsilon \downarrow 0}\left(g(t) + 2\int_t^{t+n^{1/2}h\varepsilon/c}g'(u)\, du + \{g(t)\}^{-1}\left\{\int_t^{t+n^{1/2}h\varepsilon/c}g'(u)\, du\right\}^2 g(t)\right)I\{g(t) > 0\}\\
%     &\qquad\qquad\int_{\mathcal{X}} \frac{\left\{f_{\theta_0+tc/n^{1/2}+h\varepsilon}(x)-f_{\theta_0+tc/n^{1/2}}(x)\right\}^2}{\varepsilon^2f_{\theta_0+tc/n^{1/2}}(x)}I\{f_{\theta_0+tc/n^{1/2}}(x) > 0\}\,d\mu(x)\,dt\\
%     &=\int_{-1}^1g(t)\lim_{\varepsilon \downarrow 0}\int_{\mathcal{X}} \frac{\left\{f_{\theta_0+tc/n^{1/2}+h\varepsilon}(x)-f_{\theta_0+tc/n^{1/2}}(x)\right\}^2}{\varepsilon^2f_{\theta_0+tc/n^{1/2}}(x)}I\{f_{\theta_0+tc/n^{1/2}}(x) > 0\}\,d\mu(x)\,dt
% \end{align*}
% We can get this far from the absolute continuity of $g$.}
Putting all results together, we have 
\begin{align*}
   & \sup_{|t|<1} \E^n_{\theta_0 + tc/n^{1/2}}\left\{S_n(x)-\psi(\theta_0+tc/n^{1/2})\right\}^2\\
   &\qquad\geq  \sup_{\{h:\|h\|=1\}}\lim_{\varepsilon \downarrow 0}\frac{\left\{\int_{-1}^1 \varepsilon^{-1}\{\psi(\theta_0+tc/n^{1/2})-\psi(\theta_0+tc/n^{1/2}-h\varepsilon)\}g(t)\,dt\right\}^2}{ h^T \frac{n}{c^2}\mathcal{J}(g)h + A(\varepsilon, h, q_{n,c}, f_{\theta})}
\end{align*}
where
\begin{align*}
A(\varepsilon, h, q_{n,c}, f_{\theta})
    & = \int_{-1}^1\frac{g(t+n^{1/2}h\varepsilon/c)^2}{g(t)}I\{g(t) > 0\}\\
    &\qquad\qquad\int_{\mathcal{X}} \frac{\left\{f_{\theta_0+tc/n^{1/2}+h\varepsilon}(x)-f_{\theta_0+tc/n^{1/2}}(x)\right\}^2}{\varepsilon^2 f_{\theta_0+tc/n^{1/2}}(x)}I\{f_{\theta_0+tc/n^{1/2}}(x) > 0\}\,d\mu(x)\,dt.
\end{align*}
Since the result above holds for arbitrary $h$ and $g$, we conclude the first statement by taking the supremum over $h$ and $g$ on the right-hand-side.

When \ref{as:hellinger} and \ref{as:ac_model} hold, we can apply the second statement of Lemma~\ref{lm:vtBound_directional} to the density $q_{n,c}$. Since the Fisher information of the product model at $\theta_0$ becomes $n\mathcal{I}(\theta_0)$, we have
\begin{align*}
   & \inf_{S_n}\int_{\Theta}\E^n_{\theta}\left\{S_n(x)-\psi(\theta)\right\}^2q(\theta)\, d\lambda\\
   &\qquad\geq  \sup_{\{h:\|h\|=1\}}\frac{\left\{\int_{-1}^1 \varepsilon^{-1}\{\psi(\theta_0+tc/n^{1/2})-\psi(\theta_0+tc/n^{1/2}-h\varepsilon)\}g(t)\,dt\right\}^2}{ h^T \left(\frac{n}{c^2}\mathcal{J}(g) + n\int_{\Theta} q_{n,c}(\theta) \mathcal{I}(\theta)\,d\lambda\right) h}.
\end{align*}




Let $h = M^{-1/2}u$
\begin{align*}
    h^T M h &= u^TM^{-1/2} M M^{-1/2}u= u^Tu
\end{align*}
We can simplify the second term of the denominator by the standard change of variable, 
\begin{align*}
    \int_{\Theta} q_{n,c}(\theta) \mathcal{I}(\theta)\,d\lambda = \int_{-1}^1  \mathcal{I}(\theta_0 + tcn^{-1/2})g(t)\,dt
\end{align*}
and we conclude the second claim.
\end{proof}

% \begin{proof}[\bfseries{Proof of Corollary~\ref{cor:vt_inequality}}]
% We begin with the conclusion of Theorem~\ref{thm:general_vt_inequality}. Let us consider the single observation case for a moment. By \ref{as:ac_model} that $f'_\theta(x)I\{f_\theta>0\}/\sqrt{f_\theta}$ is square-integrable almost all $\mu$ and $g$ is bounded by construction,
% \begin{align*}
%     &\lim_{\varepsilon \downarrow 0}  \frac{1}{\varepsilon^2} \int_{-1}^1\frac{g(t+n^{1/2}h\varepsilon/c)^2}{g(t)}I\{g(t) > 0\}\\
%     &\qquad\qquad\int_{\mathcal{X}} \frac{\left\{f_{\theta_0+tc/n^{1/2}+h\varepsilon}(x)-f_{\theta_0+tc/n^{1/2}}(x)\right\}^2}{f_{\theta_0+tc/n^{1/2}}(x)}I\{f_{\theta_0+tc/n^{1/2}}(x) > 0\}\,d\mu(x)\,dt\\
%     &\qquad=\int_{-1}^1\lim_{\varepsilon \downarrow 0}\frac{g(t+n^{1/2}h\varepsilon/c)^2}{g(t)}I\{g(t) > 0\}\\
%     &\qquad\qquad\int_{\mathcal{X}} \frac{\left\{f_{\theta_0+tc/n^{1/2}+h\varepsilon}(x)-f_{\theta_0+tc/n^{1/2}}(x)\right\}^2}{\varepsilon^2f_{\theta_0+tc/n^{1/2}}(x)}I\{f_{\theta_0+tc/n^{1/2}}(x) > 0\}\,d\mu(x)\,dt\\
%     &\qquad=\int_{-1}^1\lim_{\varepsilon \downarrow 0}\left(g(t) + 2\int_t^{t+n^{1/2}h\varepsilon/c}g'(u)\, du + \{g(t)\}^{-1}\left\{\int_t^{t+n^{1/2}h\varepsilon/c}g'(u)\, du\right\}^2 g(t)\right)I\{g(t) > 0\}\\
%     &\qquad\qquad\int_{\mathcal{X}} \frac{\left\{f_{\theta_0+tc/n^{1/2}+h\varepsilon}(x)-f_{\theta_0+tc/n^{1/2}}(x)\right\}^2}{\varepsilon^2f_{\theta_0+tc/n^{1/2}}(x)}I\{f_{\theta_0+tc/n^{1/2}}(x) > 0\}\,d\mu(x)\,dt\\
%     &\qquad=\int_{-1}^1g(t)\lim_{\varepsilon \downarrow 0}\int_{\mathcal{X}} \frac{\left\{f_{\theta_0+tc/n^{1/2}+h\varepsilon}(x)-f_{\theta_0+tc/n^{1/2}}(x)\right\}^2}{\varepsilon^2f_{\theta_0+tc/n^{1/2}}(x)}I\{f_{\theta_0+tc/n^{1/2}}(x) > 0\}\,d\mu(x)\,dt\\
%     &\qquad=\int_{-1}^1g(t)\int_{\mathcal{X}} \frac{\left\{f'_{\theta_0+tc/n^{1/2}}(x)\right\}^2}{f_{\theta_0+tc/n^{1/2}}(x)}I\{f_{\theta_0+tc/n^{1/2}}(x) > 0\}\,d\mu(x)\,dt \\
%     &\qquad= \int_{-1}^1 I(\theta_0 + tc/n^{1/2})g(t)\, dt
% \end{align*}
% The last equality is by Lemma~\ref{lm:dqm_and_fisher_info} assuming \ref{as:hellinger} and \ref{as:ac_model}. The proof of Lemma~\ref{lm:dqm_and_fisher_info} is analogous to Lemma 3 of \citet{gassiat2013revisiting} and provided in the appendix. Since the Fisher information at $\theta_0$ for a product model is $nI(\theta_0)$, we conclude that 
% \[\lim_{\varepsilon\downarrow0}A(h,\varepsilon, q_{n,c}, f_\theta) = n\int_{-1}^1I(\theta_0 + tc/n^{1/2})g(t)\, dt.\]
% Therefore for fixed $g$ and $h$, we have
% \begin{align*}
%     &\E^n_{\theta_0 + tc/n^{1/2}}\left[n^{1/2}\left\{S_n(x)-\psi(\theta_0+tc/n^{1/2})\right\}\right]^2 \\
%     &\qquad \geq \frac{\lim_{\varepsilon\downarrow0}\int_{-1}^1 \varepsilon^{-1}\{\psi(\theta_0+tc/n^{1/2})-\psi(\theta_0+tc/n^{1/2}-h\varepsilon)\}g(t)\,dt}{\frac{1}{c^2}\mathcal{J}(g) + \int_{-1}^1I(\theta_0 + tc/n^{1/2})g(t)\, dt}
% \end{align*}
% We thus conclude the statement of the corollary by taking the supremum over $g$ and $h$.
% \end{proof}
\begin{remark}
When $\psi$ is differentiable with respect to $\theta$ at $\theta_0$, Lemma~\ref{lm:lam_directional} recovers the standard multivariate van Trees inequality \citep{gassiat2013revisiting}.
\begin{align*}
   &\frac{\left\{\int_{-1}^1 \lim_{\varepsilon\downarrow0}\varepsilon^{-1}\{\psi(\theta_0+tc/n^{1/2})-\psi(\theta_0+tc/n^{1/2}-h\varepsilon)\}g(t)\,dt\right\}^2}{ h^T \left(\frac{n}{c^2}\mathcal{J}(g) + n\int_{\Theta} q_{n,c}(\theta) \mathcal{I}(\theta)\,d\lambda\right) h} \\&\qquad= \frac{( \partial \psi(\theta_0+tc/n^{1/2})^Th)^2}{ h^T \left(\frac{n}{c^2}\mathcal{J}(g) + n\int_{\Theta} q_{n,c}(\theta) \mathcal{I}(\theta)\,d\lambda\right) h}\\
   &\qquad = \frac{h^T\partial \psi(\theta_0+tc/n^{1/2})\partial \psi(\theta_0+tc/n^{1/2})^Th}{ h^T \left(\frac{n}{c^2}\mathcal{J}(g) + n\int_{\Theta} q_{n,c}(\theta) \mathcal{I}(\theta)\,d\lambda\right) h}
\end{align*}
We denote $\left(\frac{n}{c^2}\mathcal{J}(g) + n\int_{\Theta} q_{n,c}(\theta) \mathcal{I}(\theta)\,d\lambda\right)$ by $M$. Since the statment of Lemma~\ref{lm:vtBound_directional} holds for any $h$ such that $\|h\|=1$, we pick $h=\|M^{-1/2}\|^{-1} M^{-1/2}u$ where $u$ is a unit vector. Then 
\begin{align*}
    \frac{h^T\partial \psi(\theta_0+tc/n^{1/2})\partial \psi(\theta_0+tc/n^{1/2})^Th}{ h^T \left(\frac{n}{c^2}\mathcal{J}(g) + n\int_{\Theta} q_{n,c}(\theta) \mathcal{I}(\theta)\,d\lambda\right) h} &= \frac{u^TM^{-1/2}\partial \psi(\theta_0+tc/n^{1/2})\partial \psi(\theta_0+tc/n^{1/2})^TM^{-1/2}u}{u^TM^{-1/2}MM^{-1/2}u} \\
    &= u^TM^{-1/2}\partial \psi(\theta_0+tc/n^{1/2})\partial \psi(\theta_0+tc/n^{1/2})^TM^{-1/2}u
\end{align*}
\end{remark}
\begin{remark}
If $\psi$ is differentiable at $\theta_0$, Lemma~\ref{lm:lam_directional} recovers the standard local asymptotic minimax lower bounds as follows:
\begin{align}
   & \sup_{|t|<1} \E^n_{\theta_0 + tc/n^{1/2}}\left[n^{1/2}\left\{S_n(x)-\psi(\theta_0+tc/n^{1/2})\right\}\right]^2\geq \frac{\left\{\int_{-1}^1\frac{d}{d\theta}\psi(\theta_0+tc/n^{1/2})g(t)\, dt\right\}^2}{\frac{1}{c^2}\mathcal{J}(g)+\int_{-1}^1 \mathcal{I}(\theta_0 + tc/n^{1/2})g(t)\,dt}\nonumber\\
   &\implies\liminf_{n\to +\infty}\sup_{|t|<1} \E^n_{\theta_0 + tc/n^{1/2}}\left[n^{1/2}\left\{S_n(x)-\psi(\theta_0+tc/n^{1/2})\right\}\right]^2\geq \frac{\frac{d}{d\theta}\psi(\theta_0)^2}{\frac{1}{c^2}\mathcal{J}(g)+\mathcal{I}(\theta_0)}\label{eq:LAM_fixed_c}\\
   &\implies\liminf_{c\to +\infty}\liminf_{n\to +\infty}\sup_{|t|<1} \E^n_{\theta_0 + tc/n^{1/2}}\left[n^{1/2}\left\{S_n(x)-\psi(\theta_0+tc/n^{1/2})\right\}\right]^2\geq \frac{\frac{d}{d\theta}\psi(\theta_0)^2}{\mathcal{I}(\theta_0)}.\nonumber
\end{align}
The last expression is the classical LAM. The inequality \eqref{eq:LAM_fixed_c} is the result for LAM with a fixed local constant $c$.
\end{remark}

% % \section{Application to irregular statistical models}
% % We now consider a statistical model $\{P_\theta : \theta \in \Theta\}$ where $P_\theta$ is a collection of uniform distributions of the form $\text{Unif}[\theta-1/2, \theta+1/2]$ with the density on the real line defined as, 
% % \begin{align}
% %     f(x;\theta) = \begin{cases}
% %     1, & \text{If}\quad |x-\theta| < 1/2\\
% %     0, & \text{Otherwise}
% %     \end{cases}
% % \end{align}
% % In this problem, irregularity comes in through the statistical model, and we investigate the term $A(\varepsilon, h, q, f_{\theta})$ from Lemma~\ref{lm:vtBound_directional}.
% % % \begin{align*}
% % %     A(\varepsilon, h, q, f_{\theta}) \coloneqq \varepsilon^{-2}\iint_{\mathcal{X}\times \Theta} \frac{q(\theta+h\varepsilon)^2}{q(\theta)}\frac{\left\{f_{\theta+h\varepsilon}(x)-f_\theta(x)\right\}^2}{f_\theta(x)}I(q(\theta)f_\theta(x) > 0)\,d\mu(x)\,d\lambda.
% % % \end{align*}


% % \begin{align}
% %     \frac{\{f(x;\theta+h\varepsilon)-f(x;\theta)\}^2}{f(x;\theta)}I(f(x;\theta)>0) = \begin{cases}
% %     0, & \text{If}\quad x < \theta-\tfrac{1}{2}\\
% %     1, & \text{Else if}\quad x \in [\theta-\tfrac{1}{2}, \theta-\tfrac{1}{2}+h\varepsilon]\\
% %     0, & \text{Otherwise}.
% %     \end{cases}
% % \end{align}

% % \begin{align*}
% %     &\varepsilon^{-2}\iint_{\mathcal{X}\times \Theta} \frac{q(\theta+h\varepsilon)^2}{q(\theta)}\frac{\left\{f_{\theta+h\varepsilon}(x)-f_\theta(x)\right\}^2}{f_\theta(x)}I(q(\theta)f_\theta(x) > 0)\,d\mu(x)\,d\lambda \\
% %     & \qquad = \varepsilon^{-2}\int\frac{q(\theta+h\varepsilon)^2}{q(\theta)}\int I(x\in [\theta-\tfrac{1}{2}, \theta-\tfrac{1}{2}+h\varepsilon])\,d\mu(x)\,d\lambda\\
% %     &\qquad= \varepsilon^{-2}\int\frac{q(\theta+h\varepsilon)^2}{q(\theta)}h\varepsilon\,d\lambda \\
% %     &\qquad= \varepsilon^{-2}\int\frac{\{q(\theta+h\varepsilon)-q(\theta)+q(\theta)\}^2}{q(\theta)}h\varepsilon\,d\lambda \\
% %     &\qquad= \varepsilon^{-2}\int\frac{\{q(\theta+h\varepsilon)-q(\theta)\}^2+2q(\theta)\{q(\theta+h\varepsilon)-q(\theta)\} + q(\theta)^2}{q(\theta)}h\varepsilon\,d\lambda \\
% %     &\qquad= \int \frac{hq(\theta)}{\varepsilon} \, d\lambda+ 2\int q'(\theta+\Delta_\theta)h^2\, d\lambda +\int \{q'(\theta+\Delta_\theta)\}^2h^3\varepsilon\, d\lambda 
% % \end{align*}
% % where $\Delta_\theta \in [0, h\varepsilon]$ is a some $\theta$ dependent parameter. 


% % Another problem that might give a different result is a collection of uniform distributions of the form $\text{Unif}[0, \theta]$ with the density on the real line defined as, 
% % \begin{align}
% %     f(x;\theta) = \begin{cases}
% %     1/\theta, & \text{If}\quad x \in (0, \theta]\\
% %     0, & \text{Otherwise}
% %     \end{cases}
% % \end{align}

% % Unlike the other case, only $h=-1$ gives a meaningful result.
% % \begin{align}
% %     \frac{\{f(x;\theta-h\varepsilon)-f(x;\theta)\}^2}{f(x;\theta)}I(f(x;\theta)>0) = \begin{cases}
% %     0, & \text{If}\quad x < 0\\
% %     \frac{h^2\varepsilon^2}{\theta(\theta-h\varepsilon)^2}, & \text{Else if}\quad x \in [0, \theta-h\varepsilon]\\
% %     \frac{1}{\theta}, &\text{Else if}\quad x \in [\theta-h\varepsilon, \theta]\\
% %     0, & \text{Otherwise}
% %     \end{cases}
% % \end{align}
% % Hence we have 
% % \begin{align*}
% %     \int_0^{\theta-h\varepsilon}\frac{h^2\varepsilon^2}{\theta(\theta-h\varepsilon)^2}\, d\mu(x) + \int_{\theta-h\varepsilon}^\theta\frac{1}{\theta}\, d\mu(x) = 
% %     \frac{h^2\varepsilon^2}{\theta(\theta-h\varepsilon)} + \frac{h\varepsilon}{\theta}
% % \end{align*}


% % \begin{align*}
% %     &\varepsilon^{-2}\iint_{\mathcal{X}\times \Theta} \frac{q(\theta+h\varepsilon)^2}{q(\theta)}\frac{\left\{f_{\theta+h\varepsilon}(x)-f_\theta(x)\right\}^2}{f_\theta(x)}I(q(\theta)f_\theta(x) > 0)\,d\mu(x)\,d\lambda \\
% %     & \qquad = \varepsilon^{-2}\int\frac{q(\theta+h\varepsilon)^2}{q(\theta)}\left(\frac{h^2\varepsilon^2}{\theta(\theta-h\varepsilon)} + \frac{h\varepsilon}{\theta}\right)\,d\lambda\\
% %     &\qquad=\frac{h^2}{\theta^2} + \int\frac{q(\theta+h\varepsilon)^2}{q(\theta)} \frac{h}{\varepsilon\theta}\,d\lambda\\
% %     &\qquad = \frac{h^2}{\theta^2} + \int \frac{hq(\theta)}{\theta\varepsilon} \, d\lambda+ 2\int \frac{q'(\theta+\Delta_\theta)h^2}{\theta}\, d\lambda +\int \frac{\{q'(\theta+\Delta_\theta)\}^2h^3\varepsilon}{\theta}\, d\lambda 
% % \end{align*}
% % where $\Delta_\theta \in [0, h\varepsilon]$ is a some $\theta$ dependent parameter. 

% % \kt{To discuss}
% % Theorem 6.1 of \citet{ibragimov2013statistical} provides the lower bound of risk in terms of Hellinger distance. For the first example of $\text{Unif}[\theta-1/2, \theta+1/2]$, we have
% % \begin{align*}
% %     \int \left(\sqrt{f(x;\theta+h\varepsilon)}-\sqrt{f(x;\theta)}\right)^2\, dx = 2h\varepsilon
% % \end{align*}
% % Then we have
% % \begin{align*}
% %     \liminf_{n\to \infty}n^{-2}\left\{E_\theta(T_n-\theta)^2+E_{\theta+1/(2n)}(T_n-\theta-1/(2n))^2\right)\} > 0
% % \end{align*}

% % Here we need to use the Chapman-Robbins.
% % \begin{align*}
% %   & \inf_{S}\int_{\Theta}\E_{\theta}\left\{S(x)-\theta\right\}^2q(\theta)\, d\lambda \\
% %   &\qquad \geq  \sup_{ \|h\|<\delta}\frac{h^2}{\int_\Theta\frac{\left\{q(\theta+h)-q(\theta)\right\}^2}{q(\theta)}I(q(\theta)>0)\,d\lambda+\iint_{\mathcal{X}\times \Theta} \frac{q(\theta+h)^2}{q(\theta)}\frac{\left\{f_{\theta+h}(x)-f_\theta(x)\right\}^2}{f_\theta(x)}I(q(\theta)f_\theta(x) > 0)\,d\mu(x)\,d\lambda}.
% % \end{align*}

% % \begin{align}
% %     \frac{\{f(x;\theta+h)-f(x;\theta)\}^2}{f(x;\theta)}I(f(x;\theta)>0) = \begin{cases}
% %     0, & \text{If}\quad x < \theta-\tfrac{1}{2}\\
% %     1, & \text{Else if}\quad x \in [\theta-\tfrac{1}{2}, \theta-\tfrac{1}{2}+h]\\
% %     0, & \text{Otherwise}.
% %     \end{cases}
% % \end{align}

% % \begin{align*}
% %     &\iint_{\mathcal{X}\times \Theta} \frac{q(\theta+h)^2}{q(\theta)}\frac{\left\{f_{\theta+h}(x)-f_\theta(x)\right\}^2}{f_\theta(x)}I(q(\theta)f_\theta(x) > 0)\,d\mu(x)\,d\lambda \\
% %     & \qquad = \int\frac{q(\theta+h)^2}{q(\theta)}\int I(x\in [\theta-\tfrac{1}{2}, \theta-\tfrac{1}{2}+h])\,d\mu(x)\,d\lambda\\
% %     &\qquad= \int\frac{q(\theta+h)^2}{q(\theta)}h\,d\lambda \\
% %     &\qquad= \int\frac{\{q(\theta+h)-q(\theta)+q(\theta)\}^2}{q(\theta)}h\,d\lambda \\
% %     &\qquad= \int\frac{\{q(\theta+h)-q(\theta)\}^2+2q(\theta)\{q(\theta+h)-q(\theta)\} + q(\theta)^2}{q(\theta)}h\,d\lambda \\
% %     &\qquad= h\int q(\theta) \, d\lambda+ 2h^2\int q'(\theta+\Delta_\theta)\, d\lambda +h^3\int \{q'(\theta+\Delta_\theta)\}^2\, d\lambda 
% % \end{align*}
% % \begin{align*}
% %     \int_\Theta\frac{\left\{q(\theta+h)-q(\theta)\right\}^2}{q(\theta)}I(q(\theta)>0)\,d\lambda &=  \int_\Theta\frac{q^2(\theta+h)-2q(\theta+h)q(\theta)+q^2(\theta)}{q(\theta)}I(q(\theta)>0)\,d\lambda\\
% %     &= \int_\Theta\frac{q^2(\theta+h)}{q(\theta)}I(q(\theta)>0)\,d\lambda -2 \int_\Theta q(\theta+h)I(q(\theta)>0)\,d\lambda + 1
% % \end{align*}

% % \begin{align*}
% %     \sup_{ \|h\|<\delta}\frac{h^2}{\left(1+h\right)\int_\Theta\frac{\left\{q(\theta+h)-q(\theta)\right\}^2}{q(\theta)}\,d\lambda+2h\int\{q(\theta+h)-q(\theta)\}\,d\lambda +h}
% \end{align*}

==> main/hellinger_divergence.tex <==
\section{Minimax lower bound based on Hellinger distance}
\subsection{New bound based on van Trees inequality}
\begin{theorem}[Chapman-Robbins type van Trees inequality based on Hellinger distance]
\label{thm:crvtBound_hellinger}
Let $T$ be any vector-valued estimator  $\mathcal{X}\mapsto\mathbb{R}^s$ and $\psi$ be a functional $\Theta \mapsto\mathbb{R}^s$. Then for any $T$, for any density function $q$ that satisfies \ref{as:IPBorder} and $\|h\| < \delta$, we have
% \begin{align}
%     &\sup_{\theta\in\Theta}\E_\theta\left\{T(x)-\psi(\theta)\right\}\left\{T(x)-\psi(\theta)\right\}^T\\
%     &\qquad-
%     \frac{\int_{\Theta} \left\{\psi(\theta)-\psi(\theta-h)\right\}\left\{\psi(\theta)-\psi(\theta-h)\right\}^Tq(\theta)\,d\theta}{8-8\int_{\Theta} q^{1/2}(\theta+h)q^{1/2}(\theta)\,d\theta +4\int_{\Theta} q^{1/2}(\theta+h)q^{1/2}(\theta)H^2(P_{\theta+h}, P_{\theta})\,d\theta }\succcurlyeq 0. \nonumber
% \end{align}
\begin{align}
    &\E_\theta\left\{T(x)-\psi(\theta)\right\}\left\{T(x)-\psi(\theta)\right\}^T\nonumber\\
    &\qquad-
    \frac{\int_{\Theta} \left\{\psi(\theta)-\psi(\theta-h)\right\}\left\{\psi(\theta)-\psi(\theta-h)\right\}^Tq(\theta)\,d\theta}{4\left\{H^2(Q_h, Q) +\int_{\Theta} q^{1/2}(\theta+h)q^{1/2}(\theta)H^2(P_{\theta+h}, P_{\theta})\,d\theta\right\} }\succcurlyeq 0.
\end{align}
When $\psi$ is a real-valued functional, then the above display simplifies to 
\begin{align}
    &\inf_T\sup_{\theta\in\Theta}\E_\theta\left|T(x)-\psi(\theta)\right|^2\nonumber\\
    &\qquad\geq \sup_{\|h\|<\delta}
    \frac{\left\{\int_{\Theta} \left(\psi(\theta)-\psi(\theta-h)\right)q(\theta)\,d\theta\right\}^2}{4\left\{H^2(Q_h, Q) +\int_{\Theta} q^{1/2}(\theta+h)q^{1/2}(\theta)H^2(P_{\theta+h}, P_{\theta})\,d\theta \right\}}. 
\end{align}
\end{theorem}


\begin{theorem}[Functional analog to Theorem 6.1 of \cite{ibragimov1981statistical}]\label{thm:sharper_ihbound}
\begin{align}
     &\inf_T\sup_{\theta\in\Theta}\E_\theta\left\|T(x)-\psi(\theta)\right\|^2 \ge \sup_{\theta, \theta+h \in \Theta}\left(\frac{1 - H^2(P_{\theta + h}, P_{\theta})}{4}\right)_+\|\psi(\theta + h) - \psi(\theta)\|^2.\nonumber
\end{align}

\end{theorem}

{\color{blue}\bf Another result based on $\chi^2$-divergence. 
The chi-squared distance between $P$ and $Q$ satisfies
\[
\chi^2(P||Q) = \E_Q\left[\left(\frac{dP}{dQ} - 1\right)^2\right] \ge \sup_{\widehat{\theta}}\,\frac{(\E_P[\widehat{\theta}] - \E_Q[\widehat{\theta}])^2}{\mbox{Var}_Q(\widehat{\theta})}.
\]
Clearly, $\widehat{\theta} = \psi(P) + \widehat{\theta} - \psi(P)$ and hence $\E_P[\widehat{\theta}] = \psi(P) + b(P)$ where $b(\cdot)$ is the bias function. Therefore, with $R_{Q}(\widehat{\theta}) = \E_{Q}[(\widehat{\theta} - \psi(Q))^2]$,
\[
\chi^2(P||Q) \ge \frac{(\psi(P) - \psi(Q) + b(P) - b(Q))^2}{R_{Q}(\widehat{\theta}) - b^2(Q)},\quad\mbox{for all estimators}\quad \widehat{\theta}.
\]
Rearranging, we conclude
\begin{equation}\label{eq:main-chi-squared-bound}
R_{Q}(\widehat{\theta}) \ge b^2(Q) + \frac{(\psi(P) - \psi(Q) + b(P) - b(Q))^2}{\chi^2(P||Q)}.
\end{equation}
Swapping a roles of $P$ and $Q$, and adding the bounds, we get
\[
R_{P}(\widehat{\theta}) + R_Q(\widehat{\theta}) \ge b^2(P) + b^2(Q) + (\psi(P) - \psi(Q) + b(P) - b(Q))^2\left[\frac{1}{\chi^2(P||Q)} + \frac{1}{\chi^2(Q||P)}\right].  
\]
Define the function
\[
f(x, y) = a(b + x - y)^2 + x^2 + y^2,
\]
where $a = [\chi^{-2}(P||Q) + \chi^{-2}(Q||P)]$ and $b = \psi(P) - \psi(Q)$. Observe that
\[
\min_{x, y} f(x, y) = \frac{ab^2}{2a + 1}.
\]
This implies that
\[
\min_{\widehat{\theta}}(R_P(\widehat{\theta}) + R_Q(\widehat{\theta})) \ge |\psi(P) - \psi(Q)|^2\frac{\chi^2(P||Q) + \chi^2(Q||P)}{\chi^2(P||Q) + \chi^2(Q||P) + 2\chi^2(P||Q)\chi^2(Q||P)}.
\]
Swapping the roles of $P$ and $Q$ in~\eqref{eq:main-chi-squared-bound} and maximizing over $P, Q$, we get
\[
\max\{R_{P}(\widehat{\theta}),\, R_Q(\widehat{\theta})\} \ge \max\left\{b^2(Q) + \frac{(\psi(P) - \psi(Q) + b(P) - b(Q))^2}{\chi^2(P||Q)}, b^2(P) + \frac{(\psi(Q) - \psi(P) + b(Q) - b(P))^2}{\chi^2(Q||P)}\right\}.
\]
Now, we can define the function
\[
g(x, y) = \max\left\{y^2 + \frac{(a + x - y)^2}{\chi^2(P||Q)},\, x^2 + \frac{(a + x - y)^2}{\chi^2(Q||P)}\right\},
\]
with $a = \psi(P) - \psi(Q)$. Then
\[
\max\{R(P), R(Q)\} \ge \inf_{x, y\in\mathbb{R}} g(x, y).
\]
{\color{red}\bf What is the infimum on the right hand side?}
A simple bound can be obtained by using
\begin{align*}
g(x, y) &\ge \frac{\chi^2(P||Q)}{\chi^2(P||Q) + \chi^2(Q||P)}\left[y^2 + \frac{(a + x - y)^2}{\chi^2(P||Q)}\right] + \frac{\chi^2(Q||P)}{\chi^2(Q||P) + \chi^2(P||Q)}\left[x^2 + \frac{(a + x - y)^2}{\chi^2(Q||P)}\right]\\
&= \frac{(a + x - y)^2 + \chi^2(P||Q)y^2 + \chi^2(Q||P)x^2}{\chi^2(P||Q) + \chi^2(Q||P)}.
\end{align*}
Hence,
\begin{align*}
\inf_{x, y}\,g(x, y) &\ge \frac{1}{\chi^2(P||Q) + \chi^2(Q||P)}\,\inf_{x, y}\left[(a + x - y)^2 + \chi^2(P||Q)y^2 + \chi^2(Q||P)x^2\right]\\ 
&= \frac{a^2}{4 + \chi^2(P||Q) + \chi^2(Q||P)}. 
\end{align*}
Another alternative is to use
\begin{align*}
g(x, y) &\ge \lambda\left[y^2 + \frac{(a + x - y)^2}{\chi^2(P||Q)}\right] + (1 - \lambda)\left[x^2 + \frac{(a + x - y)^2}{\chi^2(Q||P)}\right],\quad\mbox{for}\quad \lambda\in[0, 1]\\
&= \lambda y^2 + (1-\lambda)x^2 + \left[\frac{\lambda}{\chi^2(P||Q)} + \frac{(1 - \lambda)}{\chi^2(Q||P)}\right](a + x - y)^2\\
&\ge \frac{\lambda}{1 - \lambda}\frac{a^2b^2}{(\lambda + b/(1- \lambda))^2} + b\frac{a^2\lambda^2(1-\lambda)^2}{(\lambda(1-\lambda) + b)^2}\quad\mbox{with}\quad b = \frac{\lambda}{\chi^2(P||Q)} + \frac{1-\lambda}{\chi^2(Q||P)},\\
&= \frac{\lambda(1-\lambda)a^2b^2 + ba^2\lambda^2(1-\lambda)^2}{(\lambda(1-\lambda) + b)^2}\\
&= \frac{a^2b\lambda(1-\lambda)[b + \lambda(1-\lambda)]}{(b + \lambda(1-\lambda))^2} = \frac{a^2b\lambda(1-\lambda)}{b + \lambda(1-\lambda)}.
\end{align*}
Note that $b$ is a function of $\lambda$. Now we need to optimize over $\lambda\in[0, 1]$ and this gives a better bound than both bounds derived above. 
}
\begin{figure}[h]
     \centering
     \begin{subfigure}{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/hellinger_const.png}
     \end{subfigure}
\end{figure}
\subsection{Application to local asymptotic minimax lower bounds}
\begin{corollary}\label{cor:crvt_lam_hellinger}
Theorem~\ref{thm:crvtBound_hellinger} implies 
\begin{align*}
    \liminf_{c\to +\infty}\liminf_{n\to +\infty}\sup_{\|t\|<1} \E^n_{\theta_0 + tcn^{-1/2}}\left[n^{1/2}\left\{T(x)-\psi(\theta_0+tcn^{-1/2})\right\}\right]^2\geq \nabla\psi(\theta_0)^T\mathcal{I}^{-1}(\theta_0)\nabla\psi(\theta_0).
\end{align*}
\end{corollary}

\begin{align}
   & \int_{\Theta}\E^n_{\theta}\{\widetilde{T}(x)-\widetilde{\psi}(\theta)\}^2q_{\theta_0, n,c}(\theta)\, d\theta \nonumber\\
   &\qquad \geq  \frac{\left\{\int_{\Theta} \left(\widetilde{\psi}(\theta+h)-\widetilde{\psi}(\theta)\right)q_{\theta_0, n,c}(\theta)\,d\theta\right\}^2}{4\left\{H^2(Q_h, Q) +\int_{\Theta} q_{\theta_0, n,c}^{1/2}(\theta+h)q_{\theta_0, n,c}^{1/2}(\theta)H^2(P^n_{\theta+h}, P^n_{\theta})\,d\theta\right\}}\nonumber
\end{align}
For a differentiable in quadratic mean statistical model, the above lower bound recovers the van Trees inequality. Precisely, we claim the following results:
\begin{align}
    &\lim_{\varepsilon_n\to0}\varepsilon_n^{-2}4H^2(Q_h, Q) = \frac{n}{c^2}u^T\mathcal{J}(q)u\, \text{ and}\\
    &\lim_{\varepsilon_n\to0}\varepsilon_n^{-2}4\int_{\Theta} q_{\theta_0, n,c}^{1/2}(\theta+u\varepsilon_n)q_{\theta_0, n,c}^{1/2}(\theta)H^2(P^n_{\theta+u\varepsilon_n}, P^n_{\theta})\,d\theta = nu^T\int_{\mathcal{B}_p([0],1)}\mathcal{I}(\theta_0 + tcn^{-1/2})q(t)\, dt\, u.
\end{align}

\begin{align*}
    &8-8\int_{\Theta} q_{\theta_0, n,c}^{1/2}(\theta+h)q_{\theta_0, n,c}^{1/2}(\theta)\,d\theta \\
    &\qquad= 4 \left(2-2\int_{\Theta} q_{\theta_0, n,c}^{1/2}(\theta+h)q_{\theta_0, n,c}^{1/2}(\theta)\,d\theta\right)\\
    &\qquad=4 \left(\int_{\Theta} q_{\theta_0, n,c}(\theta+h)\,d\theta+\int_{\Theta} q_{\theta_0, n,c}(\theta)\,d\theta-2\int_{\Theta} q_{\theta_0, n,c}^{1/2}(\theta+h)q_{\theta_0, n,c}^{1/2}(\theta)\,d\theta\right) \\
    &\qquad=4 \left(\int_{\Theta} \left\{g^{1/2}_{\theta_0, n,c}(\theta+h)\,d\theta- q_{\theta_0, n,c}^{1/2}(\theta)\right\}^2\,d\theta\right)\\
    &\qquad = 4 \left(\int_{\Theta} \left\{g^{1/2}\left(u+\frac{n^{1/2}h}{c}\right)-g^{1/2}\left(u\right)\right\}^2 \, du\right)
\end{align*}
We define 
\[\ell(t) = \frac{1}{2}\nabla q(t)I(q(t)>0) / \sqrt{q(t)}.\]
\kt{We need a multivariate version of Lemma 8 of \cite{pollardAsymptotia}}. 


We now set $h=u\varepsilon_n$ and let $\varepsilon_n\to0$. We then obtain 
\begin{align*}
    \varepsilon_n^{-2}\frac{4n}{c^2} \left(\int_{\Theta} \left\{\frac{g^{1/2}\left(u+\frac{n^{1/2}u\varepsilon_n}{c}\right)-g^{1/2}\left(u\right)}{n^{1/2}/c}\right\}^2 \, du\right) = \frac{n}{c^2}u^T\mathcal{J}(q)u
\end{align*}

If $\ell$ integrable such that $\int_{\mathcal{B}_p([0],1)} |\ell(t)|\, dt < \infty$
Since the Fisher information $\mathcal{J}(q) < \infty$, and $\mathcal{J}(q)=4\int_{\Theta} \ell(t)\ell(t)^T\, dt$. By Cauchy Schwarz inequality, we have
\[\]
By Lemma 8 of \cite{pollardAsymptotia} states that a nonnegative function $g$ is absolutely continuous on $\mathcal{B}_p([0],1)$ with derivative $\nabla g$. 

% \begin{align*}
%     \lim_{\varepsilon_n\to 0}\int_{\Theta} q_{\theta_0, n,c}^{1/2}(\theta+u\varepsilon_n)q_{\theta_0, n,c}^{1/2}(\theta)\, d\theta &= \int_{\Theta} \lim_{\varepsilon_n\to 0}q_{\theta_0, n,c}^{1/2}(\theta+u\varepsilon_n)q_{\theta_0, n,c}^{1/2}(\theta)\, d\theta \\
%     &= \int_{\Theta} q_{\theta_0, n,c}(\theta)\, d\theta + o(|\varepsilon_n|) \\
%     &= 1 + o(|\varepsilon_n|)
% \end{align*}

\begin{align*}
    &\lim_{\varepsilon_n\to 0}\left[8-8\int_{\Theta} q_{\theta_0, n,c}^{1/2}(\theta+u\varepsilon_n)q_{\theta_0, n,c}^{1/2}(\theta)\,d\theta +4\int_{\Theta} q_{\theta_0, n,c}^{1/2}(\theta+u\varepsilon_n)q_{\theta_0, n,c}^{1/2}(\theta)H^2(P^n_{\theta+u\varepsilon_n}, P^n_{\theta})\,d\theta\right]\\
    &\qquad =\lim_{\varepsilon_n\to 0}4\int_{\Theta} q_{\theta_0, n,c}^{1/2}(\theta+u\varepsilon_n)q_{\theta_0, n,c}^{1/2}(\theta)H^2(P^n_{\theta+u\varepsilon_n}, P^n_{\theta})\,d\theta + o(|\varepsilon_n|)\\
    &\qquad =4\int_{\Theta} \lim_{\varepsilon_n\to 0}q_{\theta_0, n,c}^{1/2}(\theta+u\varepsilon_n)q_{\theta_0, n,c}^{1/2}(\theta)H^2(P^n_{\theta+u\varepsilon_n}, P^n_{\theta})\,d\theta + o(|\varepsilon_n|)\\
    &\qquad =4\int_{\Theta} q_{\theta_0, n,c}(\theta)\lim_{\varepsilon_n\to 0}H^2(P^n_{\theta+u\varepsilon_n}, P^n_{\theta})\,d\theta + o(|\varepsilon_n|)
\end{align*}

\begin{theorem}
Theorem~\ref{thm:sharper_ihbound} implies
\begin{align}
     &\E_{\theta+h}|T-\psi(\theta+h)|^2 +\E_{\theta}|T-\psi(\theta)|^2 \ge \left(\frac{1 - H^2(P_{\theta + h}, P_{\theta})}{2}\right)_+|\psi(\theta + h) - \psi(\theta)|^2.\nonumber
\end{align}
\end{theorem}
\begin{proof}
Multiplying both sides of inequality from Theorem~\ref{thm:sharper_ihbound}, we have
\begin{align*}
    \frac{1}{2}\left(\E_{\theta+h}|T-\psi(\theta+h)|^2 +\E_{\theta}|T-\psi(\theta)|^2\right)\ge \left(\frac{1 - H^2(P_{\theta + h}, P_{\theta})}{4}\right)_+|\psi(\theta + h) - \psi(\theta)|^2.
\end{align*}
The right-hand side can be further bounded by 
\[\sup_{\|h\| < \delta} \E_{\theta+h}|T-\psi(\theta+h)|^2\ge \frac{1}{2}\left( \E_{\theta+h}|T-\psi(\theta+h)|^2 +\E_{\theta}|T-\psi(\theta)|^2\right)\]

\begin{align*}
    \frac{1 - H^2(P^n_{\theta + h}, P^n_{\theta})}{4} &= \frac{1}{4}-\frac{1}{2}\left[1-\left\{1-H^2(P_{\theta + h}, P_{\theta})\right\}^n\right]
\end{align*}
\end{proof}

\subsection{Estimation under parametric model with irregularity}
% \begin{example}
% \kt{Uniform revisited}
% Compare sharp constants in \cite{korostelev2011mathematical}.
% \begin{align*}
%     H^2(P_{\theta}^n, P_{\theta+1/n}^n) &= 2-2\left\{1-\frac{1}{2}H^2(P_\theta,  P_{\theta+h})\right\}^n
% \end{align*}


% \begin{align*}
%     H^2(P_{\theta}^n, P_{\theta+1/n}^n) &= \int \left\{\theta^{-n/2} - (\theta+1/n)^{-n/2}\right\}^2 \, dx^n\\
%     &= 2 - 2\int_0^\theta\{\theta(\theta+1/n)\}^{-n/2}\, dx^n\\
%     &= 2 - 2\int_0^\theta\{\theta^2(1+(n\theta)^{-1})\}^{-n/2}\, dx^n\\
%     &\approx 2 - 2\int_0^\theta \frac{1}{\theta^n}\{\exp(-\theta)\}^{-1/2}\, dx^n\\
%     &= 2-2\frac{1}{\exp^{1/2}(-\theta)}
% \end{align*}

% \begin{align}
%     &\inf_T\sup_{\theta\in\Theta}\E_\theta\left(T(x)-\psi(\theta)\right)^2\nonumber\\
%     &\qquad\geq \sup_{\|h\|<\delta}
%     \frac{1}{n^2\mathcal{J}(g) +4\int_{\Theta} q(\theta)\left(2-2\frac{1}{\exp^{1/2}(-\theta)}\right)\,d\theta }. 
% \end{align}
% Lower bound based on Theorem~\ref{thm:sharper_ihbound}:
% \begin{align*}
%     \left(\frac{1 - H^2(P_{\theta + 1/n}, P_{\theta})}{4}\right)_+|\psi(\theta + 1/n) - \psi(\theta)|^2 = \frac{1}{n^2} \left(-\frac{1}{4}+\frac{1}{2\exp^{1/2}(-\theta)}\right)
% \end{align*}

% \kt{According to \cite{korostelev2011mathematical}, the sharp constant is $\theta_0^2$}
% \end{example}

% \begin{example}
% $\beta$-smooth functional and $\alpha$-smooth Hellinger distance will give $n^{-2\beta/\alpha}$
% Constants

% \begin{align*}
%     \psi(\theta) = \max(0, \theta)^{1/\beta} \text{ for } \beta > 1 
% \end{align*}
% \end{example}

==> main/lam.tex <==
\section{Asymptotic properties}
\subsection{Local asymptotic minimax lower bounds} 
Let $\{P_\theta: \theta \in \Theta\}$ be a QMD statistical model with non-singular Fisher information at $\theta_0$.  Let $\psi(\theta)$ be differentiable at $\theta=\theta_0$, and $T_n$ be an estimator sequence of $\psi(\theta)$ in the model $(P_\theta^{\otimes n})$. Consider any bowl-shaped loss function $\ell: {\mathbb R}^d\rightarrow {\mathbb R}_+$. Then local asymptotic minimax theorem states that
\begin{align}
    \lim_{c \to \infty} \liminf_{n \to \infty} \sup_{\|h\| \leq 1} \E_{\theta_0 + chn^{-1/2}} \,\ell\left[n^{1/2}\left\{T_n-\psi\left(\theta_0+chn^{-1/2}\right)\right\}\right] \ge \E\,\ell(Z)
\end{align}
where $Z \sim N(0, \nabla\psi(\theta_0)^T I(\theta_0)^{-1} \nabla\psi(\theta_0))$.

\begin{enumerate}[label=\textbf{(A\arabic*)},leftmargin=2cm]
\setcounter{enumi}{3}
\item The density function $p_\theta$ is absolutely continuous over $[\theta_0 - \delta, \theta_0 + \delta]$ with gradient $\nabla p_{\theta_0}$ at $\theta=\theta_0$. For each $\theta$ in $[\theta_0 - \delta, \theta_0 + \delta]$, the function $x \mapsto \frac{1}{2}\nabla p_\theta(x)\{p_\theta(x) > 0\}/\sqrt{p_\theta(x)}$ is square-integrable with respect to $\mu$. 
\end{enumerate}
\subsection{Nonparametric efficiency bound}


==> main/motivation.tex <==
\section{}
\subsection{Limiting behaviors of $\chi^2$ divergence}
\begin{equation}
    \chi^2(P_{\theta_0} \| P_{\theta_0 + t}) = t^T I(\theta_0) t + o(\|t\|^2)
\end{equation}

==> main/nonparametric.tex <==
\section{Application to a high-dimensional problem}
\kt{Gaussian sequence model}

\begin{align*}
    Y_i = \theta_i + n^{-1/2}z_i, \quad \text{for } i = 1,2,\dots
\end{align*}
where $z_i$ are IID standard normal random variables where $\theta$ belongs to an $L_p$ ball
% \[L_p(\beta, M) = \left\{\theta:\left(\sum_{i=1}^\infty i^p|\theta_i|^p\right)^{1/p} \le M\right\}\]

==> main/van-trees-hellinger.tex <==
\newpage
\section{van Trees inequality in terms of Hellinger distance}
Recall this derivation from while ago...
\begin{align}
    &\E_{x, \theta+h} \left(T(x)-\psi(\theta)\right)\nonumber\\
    &\qquad=\iint_{\mathcal{X}\times \Theta} \left(T(x)-\psi(u-h)\right) f_u(x)q(u)\, d\mu(x)\,d\lambda(u)\nonumber\\
    &\qquad=\iint_{\mathcal{X}\times \Theta} \left(T(x)-\psi(u-h)+\psi(u)-\psi(u)\right) f_u(x)q(u)\, d\mu(x)\,d\lambda(u)\nonumber\\
    &\qquad=\E_{x, \theta}  \left(T(x)-\psi(\theta)\right)+\int_{\Theta} \left(\psi(u)-\psi(u-h)\right) q(u)\,d\lambda(u).\label{eq:remainder} 
\end{align}

\begin{align*}
    &\left|\E_{x, \theta+h}  \left(T(x)-\psi(\theta)\right)- \E_{x, \theta}\left(T(x)-\psi(\theta)\right)\right|^2 \\
    &\qquad= \left|\iint_{\mathcal{X}\times \Theta} \left(T(x)-\psi(\theta)\right)\left\{ f_{u+h}(x)q(u+h)-f_{u}(x)q(u)\right\}\, d\mu(x)\,d\lambda(u)\right|^2\\
    % &\qquad= \left|\iint \left(T(x)-\psi(\theta)\right)\left\{ f^{1/2}_{u+h}(x)q^{1/2}(u+h)-f^{1/2}_{u}(x)q^{1/2}(u)\right\}\left\{ f^{1/2}_{u+h}(x)q^{1/2}(u+h)+f^{1/2}_{u}(x)q^{1/2}(u)\right\}\, d\mu(x)\,d\lambda(u)\right|^2\\
    &\qquad\leq \iint \left(T(x)-\psi(\theta)\right)^2\left\{ f^{1/2}_{u+h}(x)q^{1/2}(u+h)+f^{1/2}_{u}(x)q^{1/2}(u)\right\}^2\, d\mu(x)\,d\lambda(u) \\
    &\qquad\qquad\iint \left\{ f^{1/2}_{u+h}(x)q^{1/2}(u+h)-f^{1/2}_{u}(x)q^{1/2}(u)\right\}^2\, d\mu(x)\,d\lambda(u)\\
    &\qquad\leq 2\iint \left(T(x)-\psi(\theta)\right)^2\left\{ f_{u+h}(x)q(u+h)+f_{u}(x)q(u)\right\}\, d\mu(x)\,d\lambda(u) \\
    &\qquad\qquad\iint  f_{u+h}(x)q(u+h)+f_{u}(x)q(u)-2f^{1/2}_{u+h}(x)q^{1/2}(u+h)f^{1/2}_{u}(x)q^{1/2}(u)\, d\mu(x)\,d\lambda(u)\\
    &\qquad= 2\iint \left(T(x)-\psi(\theta)\right)^2\left\{ f_{u+h}(x)q(u+h)+f_{u}(x)q(u)\right\}\, d\mu(x)\,d\lambda(u) \\
    &\qquad\qquad\left(2-2\iint  f^{1/2}_{u+h}(x)q^{1/2}(u+h)f^{1/2}_{u}(x)q^{1/2}(u)\, d\mu(x)\,d\lambda(u)\right)\\
    &\qquad= 2\left(\E_{x, \theta+h}  \left\{T(x)-\psi(\theta)\right\}^2 + \E_{x, \theta}  \left\{T(x)-\psi(\theta)\right\}^2\right) \\
    &\qquad\qquad\left(2-2\int q^{1/2}(u+h)q^{1/2}(u)\left\{1-\frac{1}{2}H^2(P_{u+h}, P_u)\right\}\,d\lambda(u)\right)\\
    &\qquad= 2\left(\E_{x, \theta+h}  \left\{T(x)-\psi(\theta)\right\}^2 + \E_{x, \theta}  \left\{T(x)-\psi(\theta)\right\}^2\right) \\
    &\qquad\qquad\left(2-2\int q^{1/2}(u+h)q^{1/2}(u)\,d\lambda(u) +\int q^{1/2}(u+h)q^{1/2}(u) H^2(P_{u+h}, P_u)\,d\lambda(u)\right)
\end{align*}
We thus have 
\begin{align*}
    &\frac{1}{2}\left(\E_{x, \theta+h}  \left\{T(x)-\psi(\theta)\right\}^2 + \E_{x, \theta}  \left\{T(x)-\psi(\theta)\right\}^2\right)\\
    &\qquad \geq
    \frac{\left\{\int_{\Theta} \left(\psi(u)-\psi(u-h)\right) q(u)\,d\lambda(u)\right\}^2}{8-8\int q^{1/2}(u+h)q^{1/2}(u)\,d\lambda(u) +4\int q^{1/2}(u+h)q^{1/2}(u) H^2(P_{u+h}, P_u)\,d\lambda(u)}
\end{align*}
\kt{As before, we can take $h\varepsilon_n$ for fixed $h$ i.e., direction. Then \[
\lim_{\varepsilon_n \downarrow 0}\int q^{1/2}(u+h\varepsilon_n)q^{1/2}(u)\,d\lambda(u) = 1 \]
So we have 
\[
\lim_{\varepsilon_n \downarrow 0}8-8\int q^{1/2}(u+h\varepsilon_n)q^{1/2}(u)\,d\lambda(u) = 0 \]
Further, we can assume $H^2(P_{u+h}, P_u) \lesssim |h|^\alpha$, For $n$ iid observation, we take $h\varepsilon_n = O(n^{-1/\alpha})$ such that  $H^2(P^n_{u+h}, P^n_u)$ is bounded by constant. We also assume $|\psi(u)-\psi(u-h)| \lesssim |h|^\beta$ in the ``worst" direction. Then we get $n^{-2\beta/\alpha}$ as a rate. 
}
\\
\kt{Question: How can I get a sharp constant?}
